Augmentation-Adapted Retriever Improves Generalization of Language Models as Generic Plug-In

Retrieval augmentation can aid language models (LMs) in knowledge-intensive tasks by supplying them with external information. Prior works on retrieval augmentation usually jointly fine-tune the retriever and the LM, making them closely coupled. In this paper, we explore the scheme of generic retrieval plug-in: the retriever is to assist target LMs that may not be known beforehand or are unable to be fine-tuned together. To retrieve useful documents for unseen target LMs, we propose augmentation-adapted retriever (AAR), which learns LM's preferences obtained from a known source LM. Experiments on the MMLU and PopQA datasets demonstrate that our AAR trained with a small source LM is able to significantly improve the zero-shot generalization of larger target LMs ranging from 250M Flan-T5 to 175B InstructGPT. Further analysis indicates that the preferences of different LMs overlap, enabling AAR trained with a single source LM to serve as a generic plug-in for various target LMs. Our code is open-sourced at https://github.com/OpenMatch/Augmentation-Adapted-Retriever.

==> tables/new_main.tex <==
\begin{table*}[t]
\centering
\resizebox{1.0\textwidth}{!}{%
\begin{tabular}{lll|ccccc|c}
\hline
\hline
    \multirow{2}{*}{\tf{Settings}} & \multirow{2}{*}{\tf{Methods}} & \multirow{2}{*}{\tf{\# Parameters}} & \multicolumn{5}{c|}{\tf{MMLU}} & {\tf{PopQA}} \\ & & & All & Hum. & Soc. Sci. & STEM & Other & All \\
\hline
% \tf{Vanilla LM} &&&&&& \\
Few-shot & Flan-T5$_{\text{Base}}$ & 250M & 35.8 & 39.6 & 39.8 & 26.3 & 41.2 & 8.0 \\
\hline
\multirow{4}{*}{Zero-shot} & Flan-T5$_{\text{Base}}$ & 250M & 36.1 & 40.4 & 39.8 & 27.0 & 40.6 & 8.8 \\
& Flan-T5$_{\text{Base}}$ GenRead & 250M & 34.8 & 35.1 & 34.9 & 30.6 & 39.9 & 9.1 \\
& Flan-T5$_{\text{Base}}^{\circledS}$ w/ AAR$_{\text{Contriever}}$ (Ours) & 250M & 44.4 & \tf{44.7} & \tf{47.7} & 35.8 & 52.2 & 31.9 \\
& Flan-T5$_{\text{Base}}^{\circledS}$ w/ AAR$_{\text{ANCE}}$ (Ours) & 250M & \tf{44.8} & 42.2 & 46.4 & \tf{39.0} & \tf{53.2} & \tf{37.7} \\
\hline
\hline
\multirow{2}{*}{Few-shot} & Atlas$_\text{Large}$ FT & 770M & 38.9 & 37.3 & 41.7 & 32.3 & 44.9 & n.a. \\ 
& Flan-T5$_{\text{Large}}$ & 780M & 45.1 & 47.7 & 53.5 & 34.4 & 49.2 & 9.3 \\
\hline
\multirow{4}{*}{Zero-shot} & Flan-T5$_{\text{Large}}$ & 780M & 44.8 & 46.3 & 51.4 & 34.8 & 50.6 & 7.2 \\
& Flan-T5$_{\text{Large}}$ GenRead & 780M & 42.1 & 45.0 & 48.1 & 33.6 & 45.2 & 9.1 \\
& Flan-T5$_{\text{Large}}$ w/ AAR$_{\text{Contriever}}$ (Ours) & 780M & \tf{51.8} & \tf{50.8} & \tf{59.7} & \tf{39.4} & \tf{61.8} & 33.4 \\
& Flan-T5$_{\text{Large}}$ w/ AAR$_{\text{ANCE}}$ (Ours) & 780M & 50.4 & 48.0 & 58.1 & 39.3 & 60.2 & \tf{39.3} \\
\hline
\hline
\multirow{2}{*}{Few-shot} & Atlas$_\text{XL}$ FT & 3B & 42.3 & 40.0 & 46.8 & 35.0 & 48.1 & n.a. \\ 
& Flan-T5$_{\text{XL}}$ & 3B & 51.6 & 55.0 & 61.1 & 36.8 & 59.5 & 11.1 \\
\hline
\multirow{4}{*}{Zero-shot} & Flan-T5$_{\text{XL}}$ & 3B & 51.2 & 55.5 & 57.4 & 38.1 & 58.7 & 11.3 \\
& Flan-T5$_{\text{XL}}$ GenRead & 3B & 47.4 & 51.3 & 50.2 & 34.9 & 57.4 & 11.4 \\
& Flan-T5$_{\text{XL}}$ w/ AAR$_{\text{Contriever}}$ (Ours) & 3B & \tf{56.7} & 57.7 & \tf{65.4} & \tf{43.6} & \tf{65.1} & 31.5 \\
& Flan-T5$_{\text{XL}}$ w/ AAR$_{\text{ANCE}}$ (Ours) & 3B & 56.2 & \tf{59.4} & 64.8 & 41.5 & 64.9 & \tf{38.0} \\
\hline
\hline
% \multirow{6}{*}{Few-shot} & Atlas$_\text{XXL}$ & 11B & 43.4 & 41.9 & 49.3 & 33.9 & 48.8 & n.a. \\
\multirow{1}{*}{Few-shot} & GPT-3.5 & 175B & 60.5 & 62.0 & 71.8 & 44.3 & 70.1 & 35.2 \\
% & Gopher~\cite{Gopher} & 280B & 60.0 & 56.2 & 71.9 & 47.4 & 66.1 & n.a. \\
% & Flan-PaLM~\cite{flan-t5} & 540B & 75.2 & n.a. & n.a. & n.a. & n.a. & n.a. \\
% \hline
% \tf{Fine-tuned LM} &&&&&& \\
% \hline
% UnifiedQA~\citeyearpar{2020unifiedqa} & 11B & 48.9 & 45.6 & 56.6 & 40.2 & 54.6 & n.a. \\
% \hline
% \tf{Fine-tuned LM w/ Retriever} &&&&&& \\
% \hline
\hline
\multirow{4}{*}{Zero-shot} 
& GPT-3.5 & 175B & 60.2 & \tf{65.7} & 68.0 & 46.1 & 66.5 & 34.7 \\
& GPT-3.5 GenRead & 175B & 60.0 & 63.9 & 66.5 & 48.5 & 65.7 & 38.6 \\
% \tf{Fixed LM w/ Retriever (Ours)} &&&&&& \\
% \hline
& GPT-3.5 w/ AAR$_{\text{Contriever}}$ (Ours) & 175B & 61.5 & 64.5 & \tf{73.1} & 45.0 & 69.9 & 43.9 \\
& GPT-3.5 w/ AAR$_{\text{ANCE}}$ (Ours) & 175B & \tf{62.2} & 62.0 & 72.0 & \tf{49.2} & \tf{70.7} & \tf{52.0} \\
\hline
\hline
\end{tabular}
}

\caption{
Our main results on MMLU and PopQA dataset. We group the methods mainly by the parameters. ${\circledS}$: the source LM used for training AAR; AAR$_\text{Contriever}$: AAR initialized from Contriever; AAR$_\text{ANCE}$: AAR initialized from ANCE; FT: fine-tuning; AR: adaptive retrieval. Unspecified methods represent the direct prompting. The score marked as \tf{bold} means the best performance among the models in the same setting. 
% \cx{we need to seperate zero-shot and few-shot more clearly so people make the right comparison when reading this table. Move All to the right most col under MMLU.} \cx{Don't cite Contriever ANCE in our method. It looks like it is someone else's methods} \cx{We need to discuss about the grouping of methods in this table to make the comparison more clear}
}
\label{tab:main}
\end{table*}
